Extension du formalisme des flux op\'erationnels par une alg\`ebre temporelle

Workflows constitute an important language to represent knowledge about processes, but also increasingly to reason on such knowledge. On the other hand, there is a limit to which time constraints between activities can be expressed. Qualitative interval algebras can model processes using finer temporal relations, but they cannot reproduce all workflow patterns. This paper defines a common ground model-theoretical semantics for both workflows and interval algebras, making it possible for reasoning systems working with either to interoperate. Thanks to this, interesting properties and inferences can be defined, both on workflows and on an extended formalism combining workflows with interval algebras. Finally, similar formalisms proposing a sound formal basis for workflows and extending them are discussed.

==> etc.tex <==
Je n'ai rien à dire à ce sujet pour le moment.

==> extl.tex <==
As mentionned in section~\ref{sec:wf}, disjunctions in classical workflows can depend upon conditions.
We suggest further extending workflows with the inclusion of a classical logic $\mathcal{L}$, e.g. propositional logic, yielding the language $\mathcal{W}_{\mathfrak{B},\mathcal{L}}$.

\subsection{Syntax}

$\mathcal{L}$-extended workflows are extended workflows allowing an additional flow control structure, the conditional disjunction. If $\alpha$ and $\beta$ are extended workflows and $p$ is a proposition of $\mathcal{L}$, $\miniwfcdisj{p}{\alpha}{\beta}$ is a conditional disjunction. Intuitively, if $p$ is true, workflow $\alpha$ is executed, otherwise workflow $\beta$ is executed.

The representation of figure~\ref{fig:exewf} can be completed by replacing $\miniwfdisj{\text{`garnish truffle'}}{\text{`garnish morel'}}$ with $\miniwfcdisj{\text{have\_truffle}}{\text{`garnish truffle'}}{\text{`garnish morel'}}$.

\subsection{Semantics}

The semantics of extended workflows is used as is with the following additions:

\begin{itemize}
	\item The interpretation function $\wfinterpretationfunction$ additionally maps a proposition $p \in \mathcal{L}$ to its truth value in $\proptruthvalues$;
	\item $
		\wfinterpretationof{\miniwfcdisj{p}{\varphi}{\psi}} =
			\conddef{ \wfinterpretationof{\varphi} }{ \tif \wfinterpretationof{p} = \proptrue }{ \wfinterpretationof{\psi} }{ \text{otherwise} }
		$
\end{itemize}

It is clearly the case that $\miniwfcdisj{p}{\alpha}{\beta} \not\equiv \miniwfcdisj{p}{\beta}{\alpha}$.

==> head-pres.tex <==
\usepackage{xspace,mathabx,amsmath,stmaryrd}

\usepackage{MnSymbol}
%% Redéfinir \emptyset envers et contre MnSymbol
%\DeclareSymbolFont{Symbols}{OMS}{cmsy}{m}{n}
%\DeclareMathSymbol{\emptyset}{\mathord}{Symbols}{"3B}
\renewcommand{\emptyset}{\font\cmsy = cmsy10
 \hbox{\cmsy \char 59}
}


%% table des matières automatique
\AtBeginSection[]
{
  \begin{frame}[plain]
    \tableofcontents[currentsection]
  \end{frame}
}


\def\indu{\ifmmode \mathcal{INDU} \else $\mathcal{INDU}$\xspace \fi}

\def\int#1{\llbracket#1\rrbracket}

\def\mef#1{{\huge$#1$}} % mef = mise en forme
\def\aa{\mef{\alpha}}
\def\bb{\mef{\beta}}
\def\cc{\mef{\gamma}}
\def\dd{\mef{\delta}}
\def\ee{\mef{\varepsilon}}
\def\ff{\mef{\zeta}}


\def\wfinterpretation{\omega}
\def\wftimeofeventfunction{\Theta}
\def\extwftimeofeventfunction{\Theta}
\def\wfrepetitionoperator{\uparrow}
\def\wfsequenceoperator{\to}
\def\wfinterpretationdomain{\Omega}
\def\extwfinterpretationdomain{\Omega}
\def\wfinterpretationfunction{\wfinterpretationof{\cdot}}
\def\extwfinterpretationfunction{\extwfinterpretationof{\cdot}}
%\newcommand\wfinterpretationof[1]{#1^\wfinterpretation}
\newcommand\wfinterpretationof[1]{\left\llbracket#1\right\rrbracket}
\newcommand\extwfinterpretationof[1]{\left\llbracket#1\right\rrbracket}
\newcommand\wfloop[1]{{\rcurvearrowdown}#1{\rcurvearrowup}}
\newcommand\miniwfconj[2]{\genfrac{[}{]}{0mm}{}{\displaystyle#1}{\displaystyle#2}  }
\newcommand\miniminiwfconj[2]{  \genfrac{[}{]}{0mm}{}{#1}{#2}  }
\newcommand\wfconj[2]{\left[\begin{array}{c}#1\vspace{1mm}\\#2\end{array}\right]}
\newcommand\miniwfdisj[2]{  \genfrac{\langle}{\rangle}{0mm}{}{\displaystyle #1}{ \displaystyle#2}  }
\newcommand\miniminiwfdisj[2]{  \genfrac{\langle}{\rangle}{0mm}{}{#1}{#2}  }
\newcommand\wfdisj[2]{\left\langle\begin{array}{c}#1\vspace{1mm}\\#2\end{array}\right\rangle}
\newcommand\wfsequence[2]{#1\wfsequenceoperator#2}
\newcommand\wfpsequence[2]{\left(#1\wfsequenceoperator#2\right)}
\newcommand\wftimeofevent[1]{\wftimeofeventfunction(#1)}
\newcommand\wfrepetition[2]{#1\wfrepetitionoperator#2}
%% Enlever quand \wfdisj sera utilisé partout
\def\bangle{ \atopwithdelims \langle \rangle}

\newcommand\miniwfcdisj[3]{\left\langle #1 \genfrac{}{}{0mm}{}{\displaystyle#2}{\displaystyle#3}\right\rangle }
\newcommand\miniminiwfcdisj[3]{  \genfrac{\langle}{\rangle}{0mm}{}{#1}{#2}  }

\def\induinterpretationfunction{\induinterpretationof{\cdot}}
\newcommand\induinterpretationof[1]{\left\llbracket#1\right\rrbracket}
\def\intervaldomain{\mathbb{Q}}

%\def\proptrue{\mathbf{T}}
%\def\propfalse{\mathbf{F}}
\def\proptrue{\mathtt{vrai}}
\def\propfalse{\mathtt{faux}}
\def\proptruthvalues{\{\propfalse,\proptrue\}}
\newcommand\propinterpretationof[1]{\left\llbracket#1\right\rrbracket}

\def\allenbm{\mathrel{\{b,m\}}}
\newcommand\allen[1]{\mathrel{\{\textit{#1}\}}}

\def\table{{\sc Taaable}\xspace}

\newcommand\comment[1]{\textcolor{red}{#1}}

\newcommand\conddef[4]{
	\left\{
		\begin{array}{c l}
			#1 & \quad #2 \\
     		#3 & \quad #4
  		\end{array}
  	\right.
}

\newcommand\stack[2]{ \genfrac{}{}{0mm}{0}{#1}{#2} }
\newcommand\conddefbreak[5]{
	\left\{
		\begin{array}{c l}
			#1 & \quad #2 \\
			& \quad #3 \\
     		#4 & \quad #5
  		\end{array}
  	\right.
}

%\def\tand{\text{ and }}
\def\tand{\text{ et }}
%\def\tor{\text{ or }}
\def\tor{\text{ ou }}
%\def\tif{\text{ if }}
\def\tif{\text{ si }}
%\def\totherwise{\text{ otherwise }}
\def\totherwise{\text{ sinon }}

\newcommand\sat[1]{\textsc{sat}(#1)}

\newcommand\alrel[1]{\mathrel{\{\textsf{#1}\}}}
\newcommand\alrelnb[1]{\ifmmode \mathrel{\textsf{#1}} \else \textsf{#1}\xspace \fi}

\def\wfqcninject{\mathcal{R}}

\newcommand\todo[1]{\textcolor{red}{[**#1**]}}

\def\wfint{\interpretation}
\def\qaint{\interpretation}
\def\ewfint{\interpretation}
\def\interpretation{\mathfrak{m}}
\def\qainv{\ifmmode ^\smile \else $^\smile$\xspace \fi}


% AJOUTS DE JEAN (i.e. propres, mais pas pédants)
\usepackage{tikz}
\usetikzlibrary{arrows}
\def\subsumepar{\sqsubseteq}
\def\equivalenta{\mathrel{{\subsumepar}\!\!\!\text{\reflectbox{$\subsumepar$}}}} % equivalence entre workflows
\def\langagewf{{\mathcal{W}}}
\def\langagewfe{{\mathcal{W}}_\mathfrak{B}}
\def\mlm#1{\text{\begin{tabular}{c}#1\end{tabular}}}

%\newcommand\wfconjsanscrochet[2]{\genfrac{}{}{0mm}{}{\displaystyle#1}{\displaystyle#2}}
\def\nswf{\!\!\!\!\!} %{\!\!\!\!} % negative space in workflows
\newcommand\wfconjII[2]{\left[\nswf\mlm{$\,#1\,$\\ $\,#2\,$}\nswf\right]}
\newcommand\wfconjIIsepar[2]{\left[\nswf\mlm{$#1$\\[4mm] $#2$}\nswf\right]}
\newcommand\wfconjIII[3]{\left[\nswf\mlm{$#1$\\ $#2$\\ $#3$}\nswf\right]}
\newcommand\wfconjIV[4]{\left[\nswf\mlm{$#1$\\ $#2$\\ $#3$\\ $#4$}\nswf\right]}
\newcommand\wfdisjII[2]{\left\langle\nswf\mlm{$\,#1\,$\\ $\,#2\,$}\nswf\right\rangle}
\newcommand\wfdisjIIsepar[2]{\left\langle\nswf\mlm{$#1$\\[3mm] $#2$}\nswf\right\rangle}
\newcommand\wfdisjIII[3]{\left\langle\nswf\mlm{$#1$\\ $#2$\\ $#3$}\nswf\right\rangle}
\newcommand\wfdisjIV[4]{\left\langle\nswf\mlm{$#1$\\ $#2$\\ $#3$\\ $#4$}\nswf\right\rangle}
\newcommand\wfsequenceIII[3]{#1\wfsequenceoperator#2\wfsequenceoperator#3}

\renewcommand\wfsequence[2]{#1{\wfsequenceoperator}#2}

\let\miniwfconj=\wfconjII
\let\miniwfdisj=\wfdisjII
\let\wfconj=\miniwfconj
\let\wfdisj=\miniwfdisj
\let\lien=\wfqcninject % Lien entre WF et QCN dans les EWF

\def\QCN{{N}}

% Macros de Florence :
\newcommand{\wf}{flux opérationnel\xspace}
\newcommand{\wfs}{flux opérationnels\xspace}
\newcommand{\Wf}{Flux opérationnel\xspace}
\newcommand{\Wfs}{Flux opérationnels\xspace}


==> old_sem.tex <==
%Tarski's model theory defines the semantics of a formula in terms of models. If a formula holds under the valuation provided by a model, then the model satisfies that formula. This makes it convenient to define inferences, e.g. ``$x$ implies $y$'' means that all models of $y$ are models of $x$.

\subsection{Semantics}

\subsubsection{Workflows}
\label{sec:wfsem}

A workflow represents a process definition, but each of its execution by a workflow management system and the relevant agents gives rise to a process instance. We will use the notion of process instance to build a model-theoretic semantics for the workflow formalism. The set of models of a workflow is therefore the set of process instances it can generate.

The interpretation of a workflow in a given model is an event, corresponding to a series of action instances taken by an agent to complete the workflow. The interpretation domain is the set $\Omega$ of elementary events. Non-elementary events are therefore subsets of $\Omega$. The empty set is called the impossible event, and is the only possible interpretation of unsatisfiable workflows.

An event occurs over a specific piece of time. Thus, considering a linear time that can be represented as the set of rational numbers $\mathbb{Q}$, each event can be mapped to a subset of $\mathbb{Q}$.

\paragraph{Interpretation.}
An interpretation $\wfint$ is a tuple $(\Omega, \wfinterpretationfunction, \Theta)$, where:
\begin{itemize}
	\item $\Omega$ is a non-empty set (of elementary events);
	\item $\wfinterpretationfunction$ is a function mapping a workflow $\alpha \in \mathcal{W}$ to an event $\wfinterpretationof{\alpha} \in 2^\wfinterpretationdomain$;
	\item $\wftimeofeventfunction$ is a function mapping an event $E$ to a closed and bounded set $\wftimeofevent{E} \subseteq \mathbb{Q}$ such that:
			\begin{itemize}
				\item $\wftimeofevent{\emptyset}=\emptyset$ (i.e. the impossible event does not occur);
				\item If $E\not=\emptyset$, then $\wftimeofevent{E}\not=\emptyset$ (i.e. all non-impossible events do occur);
				\item $\wftimeofevent{E \cup F} = \wftimeofevent{E} \cup \wftimeofevent{F}$ for any $E, F \in 2^\wfinterpretationdomain$ (i.e. the conjunction of two events occurs over the time when either occurs).
			\end{itemize}
\end{itemize}

A model is an interpretation of a workflow $\varphi$ if it provides a valuation such that the workflow is not mapped to the impossible event, i.e. $\wfinterpretationof{\varphi} \not= \emptyset$.

\paragraph{Conjunction.}
The conjunction of two workflows represents a complex activity with no specified constraint between the conjuncts. Therefore, the event corresponding to a conjunction is the union of the events corresponding to both, unless the interpretation of either is the empty set, in which case the conjunction cannot have a model.
\[
	\wfinterpretationof{\miniwfconj{\varphi}{\psi}} = 
	\conddef{ \wfinterpretationof{\varphi}\cup\wfinterpretationof{\psi} }{
		\tif \wfinterpretationof{\varphi} \not= \emptyset \tand \wfinterpretationof{\psi} \not= \emptyset
	}{ \emptyset }{ \totherwise }
\]

\paragraph{Sequence.}
The sequence of two workflows is a conjunction of those with an additional order constraint specifying that the first activity must be completed when the second begins. We express this constraint using a relation on the bounds of the $\Theta$s.
\[
	\wfinterpretationof{(\wfsequence{\varphi}{\psi})} =
	\conddef{ \wfinterpretationof{\varphi}\cup\wfinterpretationof{\psi} }{
			\begin{array}{l}
				\tif \wfinterpretationof{\varphi} \not= \emptyset, \wfinterpretationof{\psi} \not= \emptyset \\
				\tand \max\wftimeofevent{\wfinterpretationof{\varphi}} \leq \min\wftimeofevent{\wfinterpretationof{\psi}}
			\end{array}
	}{ \emptyset }{ \begin{array}{l} \totherwise \end{array} }
\]

\paragraph{Disjunction.}
The disjunction of two workflows has all the models of either.
\[
	\wfinterpretationof{\miniwfdisj{\varphi}{\psi}} = \wfinterpretationof{\varphi}
	\tor
	\wfinterpretationof{\miniwfdisj{\varphi}{\psi}} = \wfinterpretationof{\psi}
\]

\paragraph{Loop.}
The loop over a workflow means that the activity is repeated a number of time.
Let $\wfrepetition{\alpha}{n} = ( \dots ( \wfsequence{\alpha}{\alpha} ) \wfsequenceoperator \dots \wfsequenceoperator \alpha )$, i.e.:
\begin{itemize}
	\item $\wfrepetition{\alpha}{1} = \alpha$
	\item $\wfrepetition{\alpha}{(n+1)} = \wfsequence{ ( \wfrepetition{\alpha}{n} ) }{ \alpha }$
\end{itemize}

There exists $n \geq 1$ such that
\[
	\wfinterpretationof{ \wfloop{\varphi} } = \wfinterpretationof{\wfrepetition{\varphi}{n}}
\]

\subsubsection{Interval algebra qualitative constraints networks}
\label{sec:qasem}
Interval algebras express temporal relations between ordered pairs of formal intervals. \emph{Formal} intervals (the individuals of the language) are usually interpreted as \emph{numerical} intervals over $\mathbb{Q}$, and the relations between two numerical intervals can be formally defined as the relation between their bounds as defined in~\cite{allen81ijcai}. Interpreting formal interval as numerical intervals, it is easy to reuse those definitions to create a semantics.

\paragraph{Interpretation.}
An interpretation $\qaint$ is composed of the function $\induinterpretationfunction$ mapping a formal interval $i$ to $\induinterpretationof{i}$ a proper, closed and bounded numerical interval of $\mathbb{Q}$. A model is an interpretation of a qualitative constraint network $\mathcal{N}=(V,C)$ if it models all constraints therein:
\[
	\qaint \models \mathcal{N} \, \text{ if, for each } (V_i,V_j,C_{ij}) \in C, \, \qaint \models V_i \mathrel{C_{ij}} V_j
\]

\paragraph{Relations.}
\begin{itemize}
	\item $\displaystyle \qaint \models i \mathrel{R} j \tif \qaint \models i \mathrel{\{r\}} j \text{ for some } r \in R$;
	\item $\qaint \models i \alrel{b} j \text{ if } \max \induinterpretationof{i} < \min \induinterpretationof{j}$;
	\item $\qaint \models i \alrel{m} j \text{ if } \max \induinterpretationof{i} = \min \induinterpretationof{j}$;
	\item 
		$
		\qaint \models i \alrel{o} j \text{ if } \min \induinterpretationof{i} < \min \induinterpretationof{j},
		\max \induinterpretationof{i} > \min \induinterpretationof{j} $\\
		\phantom{$\qaint \models i \alrel{o} j \text{ if}$}		
		$
		\text{ and } \max \induinterpretationof{i} < \max \induinterpretationof{j};
		$
	\item $\qaint \models i \alrel{s} j \text{ if } \min \induinterpretationof{i} = \min \induinterpretationof{j} \text{ and } \max \induinterpretationof{i} < \max \induinterpretationof{j} $;
	\item $\qaint \models i \alrel{d} j \text{ if } \min \induinterpretationof{i} > \min \induinterpretationof{j} \text{ and } \max \induinterpretationof{i} < \max \induinterpretationof{j} $;
	\item $\qaint \models i \alrel{f} j \text{ if } \min \induinterpretationof{i} > \min \induinterpretationof{j} \text{ and } \max \induinterpretationof{i} = \max \induinterpretationof{j} $;
	\item $\qaint \models i \alrel{eq} j \text{ if } \min \induinterpretationof{i} = \min \induinterpretationof{j} \text{ and } \max \induinterpretationof{i} = \max \induinterpretationof{j} $;
	\item
		$\qaint \models i \mathrel{ \{ r\qainv \} j \tif j \mathrel{\{r\}} i }$,
		with $r\qainv$ defined by
		$\alrelnb{ p\qainv }=\alrelnb{ pi}, \alrelnb{ m\qainv }=\alrelnb{ mi},$
		\\
		\phantom{ $\qaint \models i \mathrel{ \{ r\qainv \} j \tif j \mathrel{\{r\}} i }$,}
		$\alrelnb{ o\qainv }=\alrelnb{ oi}, \alrelnb{ s\qainv }=\alrelnb{ si}, \alrelnb{ d\qainv }=\alrelnb{ di} \tand \alrelnb{f\qainv } = \alrelnb{ fi}$.
\end{itemize}

\subsection{Properties and Inferences}
\label{sec:semprop}

The semantics makes it possible to tell whether a workflow is satisfiable (i.e. there exists at least one model for $w$), and whether a workflow is more specific than another workflow (i.e. all models of $w_2$ are models of $w_1$), written $w_1 \sqsubseteq w_2$. The latter inference is used to define an equivalence relation: $w_1 \equiv w_2 \tif w_1 \sqsubseteq w_2 \tand w_2 \sqsubseteq w_1$.

It also brings to light certain properties of workflows. Specifically, the conjunction, sequence and disjunction are associative, the conjunction and disjunction are commutative, and the loop is idempotent. All those properties are modulo the equivalence. (The proofs are too cumbersome to reproduce here.)

A QCN $\mathcal{N}$ is consistent if there exists at least one solution, that is an instanciation of its variables such that all constraints are satisfied. Such a solution is equivalent to a model of $\mathcal{N}$. Finding a solution to a QCN for which a scenario is known is trivial.

The ordering of interval bounds can be exploited to find properties applicable to relation compositions. For instance, if $i\alrel{f}j$ and $j\alrel{m}k$, it can be  deduced that $i\alrel{m}k$.

